Is POS Tagging Necessary or Even Helpful for Neural Dependency Parsing?

In the pre deep learning era, part-of-speech tags have been considered as indispensable ingredients for feature engineering in dependency parsing. But quite a few works focus on joint tagging and parsing models to avoid error propagation. In contrast, recent studies suggest that POS tagging becomes much less important or even useless for neural parsing, especially when using character-based word representations. Yet there are not enough investigations focusing on this issue, both empirically and linguistically. To answer this, we design and compare three typical multi-task learning framework, i.e., Share-Loose, Share-Tight, and Stack, for joint tagging and parsing based on the state-of-the-art biaffine parser. Considering that it is much cheaper to annotate POS tags than parse trees, we also investigate the utilization of large-scale heterogeneous POS tag data. We conduct experiments on both English and Chinese datasets, and the results clearly show that POS tagging (both homogeneous and heterogeneous) can still significantly improve parsing performance when using the Stack joint framework. We conduct detailed analysis and gain more insights from the linguistic aspect.

==> content/use_bert.tex <==
\section{Integration with BERT}

\begin{table*}[htb]
\centering
\begin{tabular}{l|rrr|rrrr}
\toprule
Dataset & \#Train & \#Dev & \#Test & \#tokens & \#chars & \#POS & \#labels \\\\[-12pt]
\hline\\[-10pt]
PTB & 39,832 & 1,700 & 2,416 & 44,389 & 79 & 45 & 45 \\
CoNLL09 & 22,277 & 1,762 & 2,556 & 40,878 & 4,243 & 41 & 41 \\
CTB7 & 46,427 & 2,079 & 2,796 & 55,324 & 4,595 & 35 & 46 \\\\[-12pt]
\hline\\[-10pt]
PKU & 1,208,850 & 2,000 & 3,000 & 267,943 & 6,488 & 63 & - \\
\bottomrule
\end{tabular}
\caption{The statistics of dependency parsing and heterogeneous POS Tagging corpora.}
\label{table:statistics}
\end{table*}

Recently, the development of contextual word representations such as ELMo \cite{peters-2018-elmo} and BERT \cite{devlin-etal-2019-bert} have dramatically showed great success for many natural language processing (NLP) tasks.
Taking BERT as an example, their main idea is to train a multi-layer bidirectional Transformer \cite{vaswani-2017-attention} encoder on large-scale unlabeled texts, and use it to produce pretrained language representations.

In this paper, we take BERT as a new representation to enhance the current input features.
Since both our tagging and parsing tasks adopt word-level features, while BERT uses a more fine-grained input (subwords for English and characters for Chinese), this shows a little mismatch.
We have tried three ways: take 1) the first one, 2) the last one, 3) the average of all pieces in a word as a summary of them.
Results show that the average strategy is slightly better than the other two ways.

\citet{devlin-etal-2019-bert} compared two strategies for applying BERT to downstream tasks: the feature integration method and the finetune method, and recommended the later one.
Since what we explored are both word-level tasks, we adopt a combination of the two strategies.
Besides classifiers, we retain the word embedding and BiLSTM encoders, and feed BERT as extra feature into the BiLSTM layer.
Meanwhile, we do not freeze parameters of BERT, but finetune them during training.
Since the parameter space of BERT is huge, using it crudely can easily fall into overfitting, we apply series of regularization strategies to help improve the performance.

\subsubsection{Token Dropout} During the pretraining procedure, \citet{devlin-etal-2019-bert} introduced a so-called ``Masked LM'' strategy, which replaces the word piece with a special token randomly with a certain probability.
We retain this method at the finetuning stage \cite{Kondratyuk201975L1,clark-etal-2018-semi}.
Such special dropout strategy aims to force the model to learn a distributional contextual representation of every input token, which is critical to prevent model from overfitting and can effectively improve test performance.

\subsubsection{Layer Attention} Rather than restricted to any sublayers, we tend to collapse all BERT layers into a single vector by weighted-summation \cite{peters-2018-elmo,Kondratyuk201975L1}, called layer attention.
Specifically, assuming the intermediate output of $i^{th}$ token at $j^{th}$ BERT layer is $\mathbf{h}_{ij}$, we combine the total $L=12$ layers in the following way:
\begin{equation}
\mathbf{bert}_i^{task}=\gamma^{task}\sum_{j=1}^{L}{\mathrm{softmax}\left(\mathbf{s}_j^{task} \right) \cdot \mathbf{h}_{ij}}
\end{equation}
where $\gamma^{task}$ and $\mathbf{s}_j^{task}$ are task specific trainable weights.
We also randomly set $\mathbf{s}_j^{task}$ to $-\infty$, i.e., discard some layers to prevent the model from focusing too much on a single layer.
Once getting the BERT feature, we modify Equation \ref{eq:input} to
\begin{equation}
\mathbf{x}_i=\mathbf{e}_{w_i}^w \oplus \mathbf{bert}_i^{task}
\end{equation}
in which the tagger and parser acquire different representations, since they use separate weights corresponding to all BERT layers, and the softmax-normalized values indicate that, compared with parsing, the tagging task prefers the front layers.
Note that we directly replace the character-level model with BERT since we found the information learned by BERT has been enough and use them simultaneously doesn't make the results better.

==> source code/content/abstract.tex <==
\begin{abstract}

In the pre deep learning era, part-of-speech tags have been considered as indispensable ingredients for feature engineering in dependency parsing.
But quite a few works focus on joint tagging and parsing models to avoid error propagation.
In contrast, recent studies suggest that POS tagging becomes much less important or even useless for neural parsing, especially when using character-based word representations.
Yet there are not enough investigations focusing on this issue, both empirically and linguistically.
To answer this, we design and compare three typical multi-task learning framework, i.e., \textit{Share-Loose}, \textit{Share-Tight}, and \textit{Stack}, for joint tagging and parsing based on the state-of-the-art biaffine parser.
Considering that it is much cheaper to annotate POS tags than parse trees, we also investigate the utilization of large-scale heterogeneous POS tag data.
We conduct experiments on both English and Chinese datasets, and the results clearly show that POS tagging (both homogeneous and heterogeneous) can still significantly improve parsing performance when using the \textit{Stack} joint framework.
We conduct detailed analysis and gain more insights from the linguistic aspect.

\end{abstract}

==> source code/content/basic_model.tex <==
\section{Basic Tagging and Parsing Models}

This section presents the basic POS tagging and dependency parsing models separately in a pipeline architecture.
In order to make fair comparison with the joint models, we make the encoder-decoder architectures of the tagging and parsing models as similar as possible.
The input representation contains both word embeddings and \textsc{CharLSTM} word representations.
The encoder part adopts three BiLSTM layers.

\subsection{The Encoder Part}\label{sec:encoder-part}
\paragraph{The input layer.}
Given a sentence $S=w_0w_1 \ldots w_n$, the input layer maps each word $w_i$ into a dense vector $\mathbf{x}_i$.
\begin{equation}
\label{eq:input}
\mathbf{x}_i=\mathbf{e}_i^{w} \oplus \mathbf{e}_i^{c}
\end{equation}
where $\mathbf{e}_i^{w}$ is the word embedding, $\mathbf{e}_i^{c}$ is the \textsc{CharLSTM} word representation vector, and $\oplus$ means vector concatenation.\footnote{We have also tried the sum of $\mathbf{e}_i^{w}$ and $\mathbf{e}_i^{c}$, leading to slightly inferior performance.}
\textsc{CharLSTM} word representations $\mathbf{e}_i^{c}$ are obtained by applying BiLSTM to the word characters and concatenating the final hidden output vectors.
Following \citet{Timothy-d17-biaffine}, the word embeddings $\mathbf{e}_i^{w}$ is the sum of a fixed pretrained word embedding %from large-scale
and a trainable word embedding initialized as zero.
Infrequent words in the training data (less than 2 times) are treated as a special OOV-token to learn its embedding.
% to learn OOV embedding.
%composed of the word-level input $\mathbf{e}_{w_i}^{w}$ and character-level input $\mathbf{e}_{w_i}^{c}$. Figure \ref{fig:input} shows an illustration.

%\subsubsection{Word-level input}

%We represent the word-level input $\mathbf{e}_{w_i}^{w}$ by the sum of a pretrained vector and a learnable frequent word embedding \cite{Timothy-d17-biaffine}. Any word that occurs in the training set less than 2 times is regarded as a special OOV word.

%\subsubsection{Character-level input}

% To better leverage the word information, we also incorporate the character-level features \cite{lample-etal-2016-neural}, which has been found useful for morphologically rich languages, or to solve the data sparseness problem. Given $m$ characters $c_1c_2 \ldots c_m$ that make up the word $w_i$, we feed their corresponding trainable character embeddings into a BiLSTM encoder. The final representation is the concatenation of the last recurrent states produced by the network in respective directions, denoted by $\mathbf{e}_{w_i}^{c}$.

%\subsubsection{Independent dropout}



%After dropout, we directly take the concatenation of $\mathbf{e}_{w_i}^{w}$ and $\mathbf{e}_{w_i}^{c}$ as the entire representation.

Under the pipeline framework, the parsing model may use extra POS tags as input.
\begin{equation}
\mathbf{x}_i=\mathbf{e}_{i}^{w} \oplus \mathbf{e}_{i}^{c} \oplus \mathbf{e}_{i}^{p} \oplus \mathbf{e}_{i}^{p\prime}
\end{equation}
where $\mathbf{e}_{i}^{p}$ and $\mathbf{e}_{i}^{p\prime}$ are the embeddings of the homogeneous and heterogeneous POS tags, respectively.
For dropouts, we follow \citet{Timothy-d17-biaffine} and drop the different components of the input vector $\mathbf{x}_i$ independently.
%Assuming that there are $N$ representations, if some are dropped and the rest $M$ ones kept unchanged, we compensate them with a factor of $N/M$. For example, the compensation factor is 2 when there only exists word\&character-level input and one of them is dropped.

\paragraph{The BiLSTM encoder.} We employ the same $N=3$ BiLSTM layers over the input layer to obtain context-aware word representations for both tagging and parsing.
We follow the dropout strategy of \citet{Timothy-d17-biaffine} and share the same dropout masks at all time steps of the same unidirectional LSTM.
The hidden outputs of the top-layer BiLSTM are used as the encoded word representations, denoted as $\mathbf{h}_i$.

\subsection{The Tagging Decoder}
\label{section:tagging-decoder}

For the POS tagging task, we use two MLP layers to compute the score vector for different tags and
%We use softmax output of
get the optimal tag via softmax.
The first MLP layer uses leaky ReLU \cite{maas-2013-rectifier} activation, while the second MLP layer is linear without activation.
%$\mathbf{s}_i$ to predict the POS tag of word $w_i$.
During training, we take the local cross-entropy loss.
%objective $\mathcal{L}_{\mathrm{POS}}\left(\hat{\mathbf{t}}, \mathbf{t} \right)$, where $\hat{\mathbf{t}}$ and $\mathbf{t}$ correspond to sequences of predicted and gold tags, respectively.

%In our joint model, besides homogeneous POS tags, we also utilize additional large-scale heterogeneous data. We simply use another linear classifier after the MLP layer to predict the heterogeneous POS tags. Similarly, the objective of the heterogeneous is $\mathcal{L}_{\mathrm{POS^\prime}}\left(\hat{\mathbf{t}}^\prime, \mathbf{t^\prime} \right)$, in which $\hat{\mathbf{t}}^\prime$ and $\mathbf{t^\prime}$ are sequences of the heterogeneous.


\subsection{The Parsing Decoder}
\label{section:parsing-decoder}

%One difference between our parsing model and the basic biaffine parser is that, we replace discrete POS tags with character-level features as input. We build a stronger baseline through this modification. The remaining structure is similar to what is described in \citet{Timothy-d17-biaffine}.

We adopt the state-of-the-art biaffine parser of \citet{Timothy-d17-biaffine}.
%Specifically, like Equation \ref{eq:tag-hidden}, the parser feeds $x_i$ into the deep BiLSTM encoder, and acquires a context-aware feature vector $\mathbf{h}_i, 0\le i \le n$. Here, the $0^{th}$ position is reserved to represent the root node. Theoretically, the produced word representation retains the long-distance dependencies for word $w_i$.
%Once getting outputs from the encoder, we then apply MLP layers to these intermediate representations. Compared with previous work \cite{kiperwasser-goldberg-2016-simple}, a key observation about \citet{Timothy-d17-biaffine} is that they think the representation of a word should be different regarding whether it is a head of the directed edge or not, thus they apply different MLPs to obtain the head and dependent vector of a word respectively:
We apply an MLP layer with leaky ReLU activation to obtain the representations of each word as a head ($\mathbf{r}_i^h$) and as a dependent ($\mathbf{r}_i^d$).
\begin{equation}
%\begin{split}
%&
\mathbf{r}_i^h; \mathbf{r}_i^d =\mathrm{MLP} \left(\mathbf{h}_i \right) %\\
%& \mathbf{r}_i^d=\mathrm{MLP}^d\left(\mathbf{h}_i \right) \\
%\end{split}
\end{equation}
%where $\mathbf{r}_i^h$ is the vector of word $w_i$ as a head, and $\mathbf{r}_i^d$ as a dependent.
As discussed in \citet{Timothy-d17-biaffine}, this MLP layer on the one hand reduces the dimensionality of $\mathbf{h}_i$, and more importantly on the other hand strips away syntax-unrelated information and thus avoids the risk of over-fitting.
%in $\mathbf{r}_i$, avoiding the risk of overfitting.

Then a biaffine layer is used to %feed vectors to a biaffine layer to
compute scores of all dependencies.% via a biaffine mapping operation:
\begin{equation}
\mathrm{score}\left(i \gets j\right)=\left[
                \begin{array}{c}
                \mathbf{r}_{i}^d \\
                1
                \end{array}
              \right]^\mathrm{T}{W} \mathbf{r}_j^h
\end{equation}
where $\mathrm{score}\left(i \gets j\right)$ is the score of the dependency $i \gets j$, and ${W}$ is a weight matrix.
During training, supposing the gold-standard head of $w_i$ is $w_j$, we use the cross-entropy loss to maximize the probability of $w_j$ being the head against all words, i.e.,
$\frac{e^{\mathrm{score}\left(i \leftarrow j \right)}}
{\sum_{0 \le k \le n} e^{\mathrm{score}\left(i \leftarrow k \right)}}$.


For dependency labels, we use extra MLP and Biaffine layers to compute the scores and also adopt cross-entropy classification loss.
We omit the details due to space limitation. %We then use a similar biaffine operation to get $\mathrm{score}\left(i \gets j, l \right)$, which is the score of label $l$ assigned to dependency $i \gets j$.

%We use the softmax outputs of $\mathrm{score}\left(i \gets j\right)$ and $\mathrm{score}\left(i \gets j, l \right)$ to predict the arc $\hat{a}_i$ and its corresponding label $\hat{l}_i$. During training, we attend to compute their cross entropy objective $\mathcal{L}_{\mathrm{ARC}}\left(\hat{\mathbf{a}},\mathbf{a} \right)$ and $\mathcal{L}_{\mathrm{REL}}\left(\hat{\mathbf{l}},\mathbf{l} \right)$, where $\hat{\mathbf{a}}$ and $\hat{\mathbf{l}}$ are predicted sequences and $\mathbf{a}$ and $\mathbf{l}$ are gold ones.

==> source code/content/conclusions.tex <==
\section{Conclusions}


Unlike the findings in traditional pre-DL dependency parsing, recent studies indicate that POS tagging becomes much less important and can be replaced by \textsc{CharLSTM} word representations in neural dependency parsers.
However, there lacks a full and systematic investigation on this interesting issue, from both empirical and linguistic perspectives.
In this paper, we try to investigate the role of POS tagging for neural dependency parsing in both pipeline and joint frameworks.
We design and compare three typical joint methods based on the state-of-the-art biaffine parser.
We try to accommodate both homogeneous and heterogeneous POS tagging, considering it is much cheaper to annotate POS tags than parse trees and there exist large-scale heterogeneous POS tag datasets for Chinese.
Based on the experiments and analysis on three English and Chinese benchmark datasets, we can draw the following conclusions.
\begin{itemize}
    \item[$\bullet$] For the pipeline method, both homogeneous and heterogeneous POS tags provide little help to the basic parser with both word embeddings and \textsc{CharLSTM}, due to error propagation and the overlapping role in reducing data sparseness.
    \item[$\bullet$] The three joint methods investigated in this work perform better than the pipeline method. Among them, the \textit{Stack} is more stable and superior compared with the other three, leading to significant improvement over the basic model on all datasets.
    \item[$\bullet$] POS tagging is still helpful for dependency parsing under the joint framework even if the parser is enhanced with BERT, especially when with heterogeneous POS tagging.
    \item[$\bullet$] Detailed analysis shows that POS tagging and dependency parsing are two closely correlated tasks. In particular, If the joint model fails to resolve syntax-sensitive POS tagging ambiguities, it usually makes wrong parsing decisions as well.
\end{itemize}

%We design and compare three typical multi-task learning frameworks and results show that jointly training the POS tagging task is very helpful to parsing. We further explore the effect of the heterogeneous POS tags and find greater helpfulness compared with the homogeneous data. Detailed analysis show that our joint model brings a consistent improvement in both tagging and parsing. Our model is more capable of solving some ambiguities of POS tagging, which is crucial for improving the parsing performance. We also show that POS tagging is helpful for the strong parser enhanced with BERT....

% 试试加一下词性结果，在表格中，最后做。如果10分钟可以跑上3个结果 +BERT basic，那就跑一下



==> source code/content/exp.tex <==
\section{Experiments}

In this section, we conduct experiments and detailed analysis to make full investigation on the usefulness of POS tagging for dependency parsing.

% \input{tables/statistics.tex}
\subsection{Experimental Settings}

\paragraph{Data.} We conduct experiments on the English Penn Treebank (PTB), the Chinese dataset at the CoNLL-2009 shared task (CoNLL09) \cite{hajic-etal-2009-conll}, and the larger-scale Chinese Penn Treebank 7 (CTB7). %\cite{xue2005penn}.
For PTB, we adopt the same settings such as data split and Stanford dependencies of \citet{chen2014fast}.
We follow the official settings for CoNLL09.
% For CTB7, we use the train/dev/test data split suggested in the official document, and use StanfordParser V3???看看之前的文章怎么说。 to perform constituent-to-dependency conversion.

We use the Stanford Parser v3.0 to obtain Stanford dependencies for CTB7.\footnote{\url{https://nlp.stanford.edu/software/stanford-dependencies.shtml}}
For Chinese, besides the homogeneous POS tags, we also incorporate the large-scale People Daily corpus of Peking University (PKU) as heterogeneous POS tagging data.
% Table \ref{table:statistics} shows the statistics.

\paragraph{Evaluation metrics.} We use POS tagging accuracy (TA), unlabeled attachment score (UAS), and labeled attachment scores (LAS) for dependency parsing.
For UAS and LAS computation, We follow \citet{Timothy-d17-biaffine} and ignore all punctuation marks for PTB.
% We adopt Dan Bikel’s randomized parsing evaluation comparator for significance test.


\paragraph{Hyper-parameters.} We follow most hyper-parameter settings of \citet{Timothy-d17-biaffine} for all our models.
For \textsc{CharLSTM} word representations, we set the dimension of the character embeddings to 50, and the dimension of \textsc{CharLSTM} outputs to 100. %, same as that of the original POS tag embeddings.
%we keep the number of all BiLSTM layers to consistent 3. We set the dropout ratio of MLP for tagging to 0.5 and its output dimension is 500. The heterogeneous data is set to 10000 characters/batch.
%After back-propagation of both batches of the heterogeneous and homogeneous, we update the model simultaneously.
%Joint模型训练时，一个batch包含
%Besides the basic hyper-parameters,
%We search our hyper-parameter settings on CoNLL09 and directly apply those to the other two datasets.
We train each model for at most 1,000 iterations, and stop training if the peak performance on the dev data does not increase in 100 (50 for models with BERT) consecutive iterations.

% \paragraph{Use of BERT.}
% The recently proposed contextualized word representations, such as ELMo \cite{peters-2018-elmo} and BERT \cite{devlin-etal-2019-bert}, has been shown extremely useful for a large range of NLP tasks.
% We would like to investigate whether POS tagging is helpful for stronger parsers enhanced by BERT.
% We adopt the BERT-base model\footnote{\url{https://github.com/huggingface/transformers}} (cased for English).
% We use the word representations weighted sum of word representations of last 4 layers of BERT, denoted as $\mathbf{r}^{bert}$, as extra inputs via concatenation, i.e., $\mathbf{x}_i \oplus \mathbf{r}^{bert}$.
% During training, all BERT parameters is freezed.
% During training, we allow the model to fine-tune the BERT parameters, which we find leads to better performance than freezing BERT parameters. % when using large-scale heterogeneous POS tagging data.

% Since BERT treats the input sentences as subword (English) or character (Chinese) sequences, we use the averaged reprensentations of contained subwords/characters as word representations, which is slightly superior to previous practice of using the first or last piece.

% During training, we adopt two useful strategies to avoid over-fitting \cite{clark-etal-2018-semi,Kondratyuk201975L1}.
% First, we keep the masking operation for the BERT encoder.
% We replace the input pieces (subwords/characters) with a special token $\mathrm{[MASK]}$ with the probability of 0.2.
% Second, we randomly discard self-attention layers with the probability of 0.1 when computing $\mathbf{r}^{bert}$ via weighted sum.

% 在stack方法中，句法和词性模块使用了不同的权重，来加权求和12层表示。这个可以在加长版文章中写

%Since BERT fine-tuning requires smaller batch size and learning rate \cite{devlin-etal-2019-bert}, we set two different hyper-parameter sets for BERT and the rest parts. We set the learning rate of BERT to $5e^{-5}$, replace the input word pieces with [MASK] with a probability of 0.2, and discard some layers with a probability of 0.1 \cite{Kondratyuk201975L1}. Besides, we set 1000 characters/batch for both tagging and parsing. Largely borrowed from \citet{devlin-etal-2019-bert}'s settings, we set $\beta_1=0.9$, $\beta_2=0.99$, $\epsilon=1e^{-6}$, $weight\ decay=0.01$ for the Adam optimizer.
%fine-tune, 加一个公式 $\mathbf{x}_i \oplus \mathbf{r}^{BERT}_i$,所有字或subword的表示平均，12层加权求和，0.1的概率随机drop一层，We find a few useful tricks. token dropout，可以fine-tune，学习率降低。

\subsection{Results on the Dev Data}
%We show the main results of proposed model variants on dev data of the three datasets in Table \ref{table:dev}. Some results on PTB are missing due to the lack of English heterogeneous data.

\paragraph{Results of the pipeline framework.}
Table \ref{table:tag-dev} shows the influence of using homogeneous and heterogeneous POS tags in the pipeline framework.
More results are also presented to understand the contributions of each of the four components in the input layer.
The homogeneous tagging accuracy is 97.58, 96.59, 96.72, 97.85, on the dev data of PTB, CoNLL09, and CTB7, and PKU, respectively.
We perform 5-fold jack-knifing to obtain the automatic homogeneous POS tags on the training data to avoid closed testing, and use a POS tagger trained on PKU data to produce heterogeneous POS tags for sentences of CoNLL09 and CTB7.

The results of using only one component clearly show that lexical information (i.e., $\mathbf{e}^w$ and $\mathbf{e}^c$) is most crucial for parsing, and only using POS tag embeddings leads to very large accuracy drop.

When using two components at the same time, using \textsc{CharLSTM} word representations ($\mathbf{e}^c$) is slightly yet consistently better than using POS tag embeddings ($\mathbf{e}^p$), both substantially outperforming the model using only word embeddings ($\mathbf{e}^w$) by more than 0.5 on all three datasets.

\begin{semiwidepage}
    \begin{minipage}[tb]{0.47\textwidth}
        \centering
        \setlength{\tabcolsep}{1.5pt}
        \input{tables/tag-dev.tex}
        \captionof{table}{Parsing performance (LAS) on dev data under the pipeline framework.}
        \label{table:tag-dev}
    \end{minipage}
    \hfill
    \begin{minipage}[tb]{0.47\textwidth}
        \centering
        \setlength{\tabcolsep}{1.5pt}
        \input{tables/dev.tex}
        \captionof{table}{Parsing performance (LAS) comparison on dev data for the three joint methods.}
        \label{table:dev}
        % \vspace{0.08cm}
    \end{minipage}
    \vspace{0.5cm}
\end{semiwidepage}

Moreover, using three components leads to slight improvement on both CoNLL09 and CTB7, but hurts performance on PTB.
Further using heterogeneous tag embeddings slightly degrades the performance.

All those results indicate that under the pipeline framework, POS tags become unnecessary and can be well replaced by the \textsc{CharLSTM} word representations.
We believe the reasons are two-fold.
First, \textsc{CharLSTM} can effectively capture morphological inflections by looking at lemma/prefix/suffix, and thus plays a similar role as POS tags in terms of
alleviating the data sparseness problem of words.
Second, the error propagation issue makes predicted POS tags less reliable.


%We first investigate the influence of utilizing POS tags in different manners. \citet{dozat-etal-2017-stanfords} retained the discrete POS tag features in their parsing model, and they found a sufficiently accurate tagger is indispensable for the parsing task. However, we argue that the fixed POS tags can be completely replaced by character-based representations, and a joint model should perform better than a separate training one. To verify this, we first acquire independently trained high-quality taggers, and use them to tag the datasets, accuracies are shown in Table \ref{table:dev}. POS tags of the training set is obtained by the 5-fold cross-validation. We directly apply the predicted POS tags to the basic biaffine parser, to compare with our baseline, which uses a character-level features instead. Results are shown in Table \ref{table:tag-dev}.

%Results show that there is no significant difference between the model applying high-accurate POS tags and our baseline. Even after using the two features simultaneously, our baseline still shows competitive performance. This observation motivates us to use a joint model, and eliminate the way using predicted POS tags explicitly, which avoids suffering from the error-propagation problem.

\paragraph{Results of the joint methods.}
Table \ref{table:dev} presents the results of the three joint tagging and parsing methods without or with heterogeneous POS tagging.

When using only homogeneous POS tagging, we find that the performance gaps between different joint methods are very small.
The best joint methods outperform the basic model by 0.1, 0.3, and 0.6 respectively.
A similar situation arises when using heterogeneous tagging only.

When using both homogeneous and heterogeneous tagging , aka (w/ hetero) setting, we can see that the overall performance is further improved by large margin.
The best \textit{Stack} method outperforms the basic model by 0.6 on CoNLL09 and 0.7 on CTB7, showing that heterogeneous labeled data can inject useful knowledge into the model.

Overall, we can see that the \textit{Stack} method is more stable and superior compared with the other three methods, and is adopted for the following experiments and analysis.

% 词性和句法任务紧密相关，大部分词性消歧都可以看成是句法的子任务，被句法覆盖，因此同构词性的loss其实基本都被句法的loss覆盖了。因此同构词性的作用一般不大。


%We compare the tagging accuracies of our joint models with that of the baseline, as shown in Table \ref{table:dev}. Since the baseline model does not contain a POS tagging part, we report the results produced by the taggers trained separately as benchmarks.
%For the direct MTL framework, the joint models show no noteworthy improvements, and even hurt the performance on PTB dataset. After adding heterogeneous POS tags, the accuracies increase by about 0.3 on the two Chinese datasets. This indicates that, to some extent, the heterogeneous data brings separate features for the tagging model, which is implicitly helpful to the homogeneous tagging.

%\subsubsection{Results of parsing.}

%Scores of dependency parsing are also available in Table \ref{table:dev}. We can see that the joint model brings substantial improvements over the baseline by 0.3 or 0.6 regarding whether heterogeneous POS tags are used. There exist slight improvements on PTB, possibly because the results of baseline are good enough and the heterogeneous data is lacking.

%Specifically on all model variants, there are subtle differences in the results. The Stack approach achieves best performances in general. We argue that this is because the intermediate representations learned by Stack can capture more implicit information of POS tags than Stack-Discrete, which uses discrete POS tags instead. Share-Loose shows uncompetitive results, possibly due to the poor relevance of the two sub-models for respective tasks, especially compared with the tightly model Share-tight.

\subsection{Final Results on the Test Data}

\input{tables/final.tex}

Table \ref{table:final-results} shows the results on the test data.
For the scenario of not using BERT, the pipeline method using homogeneous POS tags is slightly yet consistently inferior to the basic model.
The \textit{Stack} method using only homogeneous POS tags significantly outperforms the basic method by 0.2 ($p<0.005$), 0.4 ($p<0.0005$), and 0.5 ($p<0.0005$) in LAS on the three datasets respectively.
Utilizing heterogeneous POS tags on Chinese further \textcolor{black}{boosts} parsing performance, leading to large overall improvements of 0.9 ($p<0.0001$) on both datasets.

When using BERT, parsing accuracy of the basic method increases by very large margin.
%0.8, 3.4, and 3.4 respectively.
Compared with the stronger baseline, the improvement introduced by POS tagging becomes smaller.
Overall, using both homogeneous and heterogeneous POS tagging, the \textit{Stack} method significantly outperforms the basic method by 0.3 ($p<0.005$) on both CoNLL09 and CTB7.


%Combined with the results on dev data, we directly apply BERT to the best performing Stack model. Final summary results on test datasets are reported in Table \ref{table:final-results}. We first reproduce the results reported in \citet{Timothy-d17-biaffine}, and LAS of our implementation on CoNLL09 is 85.53, similar to that in the paper (85.38). The result of our baseline (86.00), is superior to the basic biaffine parser. This proves that replacing the tag embeddings with character-level representations can effectively solve the error propagation problem.

%The joint model achieves absolute improvements of 0.2 ($p<0.005$) on English PTB, 0.4 and 0.5 ($p<0.0005$) on the two Chinese datasets respectively. We further apply heterogeneous data on Chinese, leading to an overall improvement of 0.9 ($p<0.0001$).
%Even after incorporating BERT, our method still increase LAS by 0.3 ($p<0.005$) on the basis of strong baseline, which again indicates the significant helpfulness of heterogeneous POS tags.

For POS tagging, the trend of performance change is similar.
First, the joint method can also improve tagging accuracy, especially when with heterogeneous POS tagging.
Using Bert can substantially improve TA on both Chinese datasets.
However, it is surprising to see a slight decrease in TA when using BERT, which is possibly due to over-fitting considering the TA is already very high on English.

We also list the results of recent previous works.
We can see that our final joint models achieve competitive parsing accuracy on PTB and CoNLL09 w/ or w/o BERT. %\textcolor{red}{CTB7是不是需要说一下。}
% scenarios.
% Our results have exceeded most predecessors' work and achieved the state-of-the-art performance.

\subsection{Detailed Analysis}
In the following, we conduct detailed analysis on the CoNLL09 test data, in order to understand or gain more insights on the interactions and mutual influence between POS tagging and dependency parsing.
For the joint method, we adopt the \textit{Stack} model with both homogeneous and heterogeneous POS tagging without using BERT, to jointly produce automatic POS tags and parse trees.
For the pipeline method, we use the two basic tagging and parsing models separately to produce automatic results.
%96.42
%96.66 (joint)
%To find out the factors in POS tagging that have the greatest impact on syntactic performance, we conduct detailed gap analysis through comparing the results of our baseline and the joint model on CoNLL09 test set.
\begin{figure}[tb]
\centering
\includegraphics{figures/tp-bar.pdf}
\caption{Changes of tagging accuracy and parsing accuracy (LAS) on the CoNLL09 test set for words of different POS tags. Words/arcs are categorized according to their/their dependent's gold-standard POS tags.}
\label{fig:tp-bar}
\end{figure}

\paragraph{Correlation of performance changes between tagging and parsing.}
Overall, the joint method outperforms the pipeline method by 0.2 in TA, and 0.7/0.9 in UAS/LAS, as shown in Table \ref{table:final-results}.
To gain more insights, we categorize all words according to their gold-standard POS tags and compare the accuracy changes for each set.
Figure \ref{fig:tp-bar} shows the most frequent tags. % in the descending order of frequency.
We can see that there is clear positive correlation of absolute performance changes between tagging and parsing.
For instance, as the most frequent tags \texttt{NN} and \texttt{VV}, their tagging accuracy increases by 0.2 and 0.7, and parsing accuracy increases by 0.7 and 1.4, respectively.
The most notable exception is \texttt{NR} with opposite changes in tagging and parsing accuracy (-0.6 vs. +1.3), which can be explained from two aspects.
First, we find that most of \texttt{NR} mistakes are due to the \{\texttt{NR}, \texttt{NN}\} ambiguous pair, which is syntax-insensitive and thus has very small impact on parsing decisions.
Second, the \textit{Stack} model may be more robust to tagging errors.

Overall, we conclude that tagging and parsing performance is highly correlated due to the close relationship between the two tasks.
% In order to gain more We classify compare the results of the joint and pipeline models
%NN->JJ UAS: 91.96
%JJ->NN UAS: 92.82
%Figure \ref{fig:tp-bar} shows the changes of tagging and parsing results classified by POS tag types. We select the most frequent and prominent POS tags from the tag set and rank them in descending order. We then list the improvements on both tagging and parsing according to each POS tag in the figure.
%Especially, we argue that the tagging task can be understood as sub-task.
%We can see that both the improvements of tagging and parsing show a consistent trend regarding different POS tags in general. Though not explicitly used in the joint model, the correct prediction of some tags can still bring tremendous improvement to syntax parsing. A notable example is that, predicting the tag JJ correctly brings about a 2.6 improvement in parsing. Moreover, the result of tagging on JJ also increases about 1.6, which indicates the two tasks can promote each other.

\paragraph{Influence of tagging errors on parsing.}
%Though the Stack method does not explicitly use the predicted POS tags from the tagging component,
In the \textit{Stack} method, the hidden representations from the tagging encoder is fed into the parsing encoder as extra inputs.
We would like to understand how tagging decisions influence parsing.
Overall, UAS/LAS are 90.42/88.38 for words getting correct POS tags, whereas 73.40/42.59 for wrongly tagged words.
We can observe dramatic drop of 17.0/45.8, indicating that POS tags has much larger influence on LAS than UAS.
\input{tables/tag-pair.tex}

Looking deeper into this issue, Table \ref{table:tag-pair} shows the parsing accuracy for words of different POS tagging patterns.
A tagging pattern \texttt{X} $\rightarrow$ \texttt{Y} represents the set of words whose correct tag is \texttt{X} and \textcolor{black}{are} tagged as \texttt{Y}.

We can see that higher parsing accuracy are usually achieved by correct tagging patterns \texttt{X} $\rightarrow$ \texttt{X} than wrong pattern \texttt{X} $\rightarrow$ \texttt{NOT-X}, except %the only exception of
\texttt{DEC} $\rightarrow$ \texttt{DEG} in UAS.\footnote{\texttt{DEG} and \texttt{DEC} are two tags for the frequently used auxiliary word ``的'' ($\mathrm{d\bar{e}}$, translated as ``of'' or ``that'') in Chinese. ``的'' is tagged as \texttt{DEG} in phrase ``土地/land 的 面积/area (area of the land)'', while as \texttt{DEC} in ``他/he 提出/proposed 的 方法/method (method that he proposed)''.}.

The tagging ambiguites can be classified into three types.
First, the syntax-sensitive ambiguous pairs such as \{\texttt{NN}, \texttt{VV}\} and \{\texttt{VV}, \texttt{AD}\} lead to large performance decrease in both UAS and LAS if wrongly tagged.
Second, the syntax-insensitive ambiguous pairs such as \{\texttt{NN}, \texttt{NR}\} and \{\texttt{VV}, \texttt{VA}\} have very small influence on parsing accuracy.
Finally, some ambiguous pairs only greatly influence LAS but have little effect on UAS, such as \{\texttt{NN}, \texttt{JJ}\} and \{\texttt{DEC}, \texttt{DEG}\}.

%There are some tags with abnormal results in Figure \ref{fig:tp-bar}, however, which violate the above trend, e.g., NR and CD. The tagging result on NR decreases about 0.6 but the parsing result increases about 1.3, while the opposite phenomenon appears on CD. To investigate this, we further analyse the impact of tagging on parsing task, as shown in Table \ref{table:tag-pair}.
% In our statistics, the most likely error pair on NR is \{\texttt{NR}, \texttt{NN}\}, which act similar syntactic roles for parsing,


%In the table, we list the most typical tagging pairs of some frequent POS tags and their corresponding parsing results. We can see some error pattern of POS tags, like \{\texttt{NN}, \texttt{JJ}\}, \{\texttt{VV}, \texttt{AD}\} and \{\texttt{DEG},\texttt{DEC}\}, can heavily affect the parsing. Taking \{\texttt{DEG},\texttt{DEC}\} as a case study, the parsing performance achieves 95.91 once the tag is correctly predicted, and drops dramatically to 26.56 when mispredicted as DEC \footnote{DEG and DEC are always used as the annotations for two Chinese auxiliary words ``的'' or ``之'', but have subtle difference. ``的'' is tagged as DEG in phrase ``主要/primary 的 工作/work (primary work)'', while as DEC in ``举行/hold 的 比赛/competition (held competition)''.}. We argue that the processing of such confusing POS tag is crucial to the construction of syntactic structure. Our joint model is more capable of handling such ambiguous pairs and can bring significant improvement on specific mode.

%\subsubsection{Impact of POS tags as heads or dependents}

% We inspect the parsing results regarding to the POS tags as heads or dependents, from both arc (UAS) and relationship (LAS) perspectives, as shown in Table \ref{table:tag-overall}.

% From the table, we can see the UAS increases by 31.00 if the POS tags is correctly predicted as heads, but only 17.02 as dependents. This shows that the tags on heads play more important roles on the arc prediction.

% In contrast, The second major row in the table shows that POS tags as dependents may be more important in predicting relationships, in which the results increase by 44.54 and 45.79 regarding whether as heads or dependents respectively.

% In general, our joint model is better than the baseline in dealing with some POS tag ambiguity, which is crucial from parsing viewpoint.

==> source code/content/introduction.tex <==
\section{Introduction}
\input{figures/instance.tex}
% AAAI论文需要对背景介绍更多：
%In the research field of natural language processing,
Among different NLP tasks, syntactic parsing is the first to convert sequential utterances into full tree structures.
Due to its simplicity and multi-lingual applicability, dependency parsing has attracted extensive research interest as a main-stream syntactic formalism \cite{nivre-lrec2016-UD1.0,zeman-etal-2018-conll}, and been widely used in semantic parsing \cite{hajic-etal-2009-conll}, information extraction \cite{roller-etal-2018-hearst}, machine translation \cite{%wu-etal-2017-sequence,
zhang-etal-2019-syntax}, etc.

% srl：可以引用庆荣的文章

Given an input sentence $S=w_0w_1 \ldots w_n$,
%the goal of
dependency parsing constructs a tree
$T=\{(h,d,l), 0\le h \le n, 1 \le d \le n, l \in \mathcal{L}\}$,
as depicted in Figure \ref{fig:example-dep},
where $(h,d,l)$ is a dependency from the head $w_h$ to the dependent $w_d$ with the relation label $l$, % \in \mathcal{L}$,
and $w_0$ is a pseudo root node.
%Given an input sentence, the goal of dependency parsing is to represent its syntactic structure as a dependency tree, as depicted in Figure \ref{fig:instance}.
% 加一句话，一个例子（有两种词性），介绍依存句法分析的重要意义。

% Introduction目前太长，我会简写，压缩内容。有些内容会放到related work部分。

In the pre deep learning (DL) era, part-of-speech (POS) tags are considered as indispensable ingredients for feature engineering in dependency parsing.
POS tags function as word classes in the sense that the same POS tags usually play similar syntactic roles in language utterances.
For example, ordinary verbs are tagged as \texttt{VV} and ordinary nouns as \texttt{NN} in Penn Chinese Treebank (CTB).
Yet some tags are designed for serving other tasks such as information extraction.
For instance, proper nouns and temporal nouns are distinguished from \texttt{NN} as \texttt{NR} and \texttt{NT} respectively.
In this sense, we refer to tag pairs like \{\texttt{NN},\texttt{VV}\} as syntax-sensitive and \{\texttt{NN},\texttt{NR}\} as syntax-insensitive.
%As a pre-processing step of syntax annotation, POS tags
%as a shadow syntactic syntactic information
%effectively
%function as word classes in the sense that words with the same POS tag usually play similar syntactic roles in language utterances. For example,
%\footnote{Sometimes fine-grained tags are distinguished for morphological analysis (e.g. singular \texttt{NN} vs. plural NNS in English Penn Treebank) or for better serving information extraction (e.g., \texttt{NN} for ordinary noun vs. NNP for proper noun).
%Plural (NP NNPS). Morphological features.
%}
%https://www.ling.upenn.edu/courses/Fall_2003/ling001/penn_treebank_pos.html
Parsing performance drops dramatically when removing POS-related features, since
%Therefore,
POS tags play a key role in reducing the data sparseness problem of using pure word-based lexical features.
%than removing word-related features in a traditional dependency parser (CITE).
Meanwhile, to alleviate error propagation in the first-tagging-then-parsing pipeline,
researchers propose to jointly model POS tagging and dependency parsing under both graph-based \cite{li-etal-2011-joint} and transition-based \cite{hatori-etal-2011-incremental} frameworks. %, leading to substantially better tagging and parsing performance.


%词性对于传统离散特征的句法分析非常重要，解决词特征的数据稀疏问题，indispensable
%很多工作研究词性和句法联合，结果很好



In the past five years, dependency parsing has achieved tremendous progress thanks to the strong capability of deep neural networks in representing word and long-range contexts \cite{chen2014fast,dyer-etal-2015-transition,zhou-etal-2015-neural,andor-etal-2016-global,kiperwasser-goldberg-2016-simple,Timothy-d17-biaffine}.
Yet all those works hold the assumption of POS tags being important and concatenate word and POS tag embeddings as input.

% In the first successful neural dependency parser of \citet{chen2014fast}, POS tags are used as important atomic features in a similar manner as in traditional discrete-feature based parsing.
% As a transition-based parser, a simple feed-forward network is used for action scoring, with non-linear activation functions for automatically combining atomic features.
% They employ greedy search to determine the optimal action sequence, which is further extended with beam search by Zhang et al., (2015) and Andor et al., (2016).
% Dyer et al. (2015) proposed stack LSTM to better encode the partially generated partial trees in the stack without using explicit atomic features, leading to ....
% \citet{kiperwasser-goldberg-2016-simple} utilize BiLSTM as an encoder and achieve excellent results in both graph-based and transfer-based parsers. Based on this work, \citet{Timothy-d17-biaffine} propose a simple yet effective deep biaffine graph-based parser and achieve the state-of-the-art accuracy on a variety of datasets and languages.

Moreover, researchers show that using Character-level Long Short-term Memory (\textsc{CharLSTM}) based word representations is helpful for named entity recognition \cite{lample-etal-2016-neural}, dependency parsing \cite{dozat-etal-2017-stanfords}, %che-etal-2018-towards}
and constituency parsing \cite{kitaev-klein-2018-constituency}. %can further improve parsing performance.
The idea is first to perform Long Short-term Memory (LSTM) over word characters and then to add (or concatenate) together word embeddings and \textsc{CharLSTM} word representations as model inputs.
In particular, \citet{kitaev-klein-2018-constituency} show that with \textsc{CharLSTM} word representations, POS tags are useless for constituency parsing.
We believe the reason may be two-fold.
First, word embeddings, unlike lexical features, suffer from much less data sparseness, since syntactically similar words can be associated via similar dense vectors.
Second, \textsc{CharLSTM} word representation can effectively capture morphological inflections by looking at lemma/prefix/suffix, which provide similar information as POS tags.
However, there still lacks a full and systematic study on the usefulness of POS tags for dependency parsing.

In this work, we try to answer the question whether POS tagging is necessary or even helpful for neural dependency parsing
and make the following contributions\footnote{We release our code at \url{https://github.com/Jacob-Zhou/stack-parser}.}.
%from the following aspects. （有点怪）
\begin{itemize}
\item[$\bullet$] We design three typical multi-task learning (MTL) frameworks (i.e., \textit{Share-Loose}, \textit{Share-Tight}, \textit{Stack}), for joint POS tagging and dependency parsing based on the state-of-the-art biaffine parser.
\item[$\bullet$] Considering that there exist large-scale heterogeneous POS-tag data for Chinese partly because it is much cheaper to annotate POS tags than parse trees, we also investigate the helpfulness of such heterogeneous data, besides homogeneous POS-tag data that are annotated together with parse trees.
\item[$\bullet$] We conduct experiments on both English and Chinese benchmark datasets, and the results show that POS tagging, both homogeneous and heterogeneous, can still significantly improve parsing accuracy when using the \textit{Stack} joint framework.
Detailed analysis sheds light on the reasons behind helpfulness of POS tagging.
\end{itemize}

%asked in the paper title and make a full and systematic study on this issue, this paper makes the following contributions.




%哪些工作开始用\textsc{CharLSTM}词表示？(ELMo?)看一看啊。
%Under the graph-based framework,

%然而神经网络模型中，早期还是要使用词性。后面就发现词性越来越不重要，只要通过lstm或sa得到句子长距离依赖信息，就可以绕过词性。

% 这些工作的出发点都是，word embedding把词看成基本单元，不同的词对应不同的向量，虽然可以通过训练，让相似的词的向量更相似。但是没有利用词本身的构词信息，即词根、词干、词缀等提供的信息，这些信息可以从另一个角度，更便捷的把不同的词联系在一起。
% 而利用词根、词干等信息，对于词性标注本身也很重要。

% 词性可以分为两种，对句法有关系的词性细化，与句法无关的词性细化。从前一个角度看，词性可以认为是句法的一个子、简化任务。如果有了句法信息，前一类词性消歧问题通常直接就可以解决。
% 从后一类词性细化角度看，词性和句法关系不大，但是对句法的影响也不太大，是否做对影响也不大。

% 这也是为什么同构词性数据集的作用不太大。异构词性数据集作用更大，是因为数据更多了。异构数据集由于测试集本身的偏置（biase），比汇报的性能应该更大。

% 词性和句法的影响的工作：stack-propagation，conll-2018等

% 为什么加了同构没有用。因为句法是词性的一个超集，可以根据句法推理触大多数词性歧义。

% 词性实际已经不是必须的了。

%% 一个IDEA：如果词性作用不大了，那么是否使用粗糙词性集合（Universal POS tag, 14种词性。我觉得以后就应该用非常粗糙的词性集合。Noun和Verb不容易区分时就专门弄一个标签，或者直接标注为两者即可。属于词法上的分析，以后也不要再标注词性数据了。只要在词典上标注词性信息即可。




==> source code/content/joint_model.tex <==
\section{Joint Tagging and Parsing Models}

\begin{figure*}[tp]
\begin{widepage}
\centering
\includegraphics[scale=0.7]{figures/framework.pdf}
\end{widepage}
\caption{The framework of three variants of the joint model.}
\label{fig:framework}
\end{figure*}

%This section gives a detailed description of our joint model for POS tagging and dependency parsing, and clarifies the way of exploiting large-scale heterogeneous data to help boost the performance. We first present the inference procedure of each model component. Then, we explore the different manners of their combination by introducing three variants. Finally, on the best one, we also apply BERT, further confirming the effectiveness of our joint model.

%After a detailed discussion of the individual tagging and parsing part, in this section, based on previous work, we tend to combine them for MTL, verifying the helpful role of POS Tagging in the parsing task. The heterogeneous POS tagging is also covered in our joint model. We have tried three variants of the joint model to find out which one can make better use of POS tags, as explained below. Figure \ref{fig:framework} shows their frameworks.

The pipeline framework suffers from the error propagation problem, meaning that POS tagging mistakes badly influence parsing performance.
In the pre-DL era, researchers propose joint tagging and parsing models under both graph-based and transition-based parsing architectures \cite{li-etal-2011-joint,hatori-etal-2011-incremental}.
The key idea is to define the joint score of a tag sequence and a parse tree and to find the optimal joint result in the enlarged search space.
In the neural network era, jointly modeling two tasks becomes much easier thanks to the commonly used encoder-decoder architecture and the MTL framework.

In this work, we design and compare three typical MTL frameworks for joint POS tagging and dependency parsing, i.e., \textit{Share-Loose}, \textit{Share-Tight}, and \textit{Stack}, as illustrated in Figure \ref{fig:framework}.
The \textit{Share-Loose} and \textit{Share-Tight} methods treat tagging and parsing as two parallel tasks, whereas the \textit{Stack} method consider parsing as the main task and derive POS tag-related information as the inputs of the parsing component. For all joint models, the inputs only include the word embeddings and \textsc{CharLSTM} word representations, as shown in Equation \ref{eq:input}.

\paragraph{Share-Loose.}
The tagging and parsing tasks use nearly separate networks, and only share the word and char embeddings.
To incorporate heterogeneous POS tagging data, we add another scoring MLP at the top to compute scores of different heterogeneous POS tags.
%The tagger is used to learn both the homogeneous and heterogeneous tags.
%In such loosely joint model, the two tasks have an implicit influence on the other one.
Under such architecture, the loosely connected tagging and parsing components can only influence each other in very limited manner.

\paragraph{Share-Tight.} This is the most commonly used MTL framework, in which the tagging and parsing components share not only the embeddings, but also the BiLSTM encoder.
Different decoders are then used for different tasks.
%Once getting the outputs from the encoder, we employ different components, as described in Section \ref{section:tagging-component} and Section \ref{section:parsing-component}, for respective tasks.
%In this tightly joint model, the tagging task acts as regularization of parsing.
In this tightly joint model, the tagging and parsing components can interact with and mutually help each other to a large extent.
The shared parameters are trained to capture the commonalities of the two tasks.

% Note that although similar in naming, the variants Share-Loose and Share-Tight are not identical in basic structure compared with the joint models proposed by \citet{straka-2018-udpipe}, we just borrowed their names. NEED to 搞清楚这个文章干啥了，得说清楚。related work部分也得写。
% Tagger Parser，有shared LSTM，也有私有的LSTM。
% \textcolor{red}{CoNLL 2018 UD Shared
% Task: Multilingual Parsing from Raw Text
% to Universal Dependencies,包含sentence segmentation, tokenization,POS tagging, lemmatization和dependency
% parsing，lemmatization作为词性网络中UPOS,XPOS和UFeats之外的第四种，词性句法联合训练，tight和loose，tight部分除了共享的LSTM之外还有分开的LSTM}

% 需要仔细检查一下，最好统一一下framework, model, architecture的用词。


% \textbf{Stack-Discrete.}
% Different from the Share-Loose/Tight methods, the Stack-Discrete method uses shared word and char embeddings and separate BiLSTM encoders for the tagging and parsing tasks.
% Most importantly, the parsing component takes the discrete 1-best POS tag predicted by the tagging component as extra inputs, similarly to the pipeline framework.
% For example, if the tagging component predict ``NN'' as the max-scoring tag of $w_i$, we feed the corresponding tag embedding of ``\texttt{NN}'', denoted as $\mathbf{e}^p_i$, as extra input of the BiLSTM encoder of the parsing component.
%, represented by.
% \begin{equation}
% % \mathbf{x}_i=\mathbf{e}_i^w \oplus \mathbf{e}_i^c \oplus \mathbf{r}_i^p
% \mathbf{x}^{parse}_i = \mathbf{x}_i \oplus \mathbf{e}_i^p
% \end{equation}
% We argue that this method can alleviate (though still suffers from) the error propagation problem to some extent, since the tagging and parsing components are jointly trained and adapted to becoming more robust.

%the online predicted 1-best POS tag

%Please kindly note that
% The idea behind the {Stack-Discrete} joint method is borrowed from \citet{nguyen-verspoor-2018-improved}.
% They show that the joint method can greatly improve parsing performance of the BIST parser based on BiLSTM encoder \cite{kiperwasser-goldberg-2016-simple}, and achieves an LAS of 92.87 on PTB.
% In this work, we use the {Stack-Discrete} joint method as a representative approach and try to make thorough investigations based on the state-of-the-art biaffine parser.

% as their baseline and show that the joint
% 什么语言上做的实验，baseline是什么，结果如何。
% \textcolor{red}{词性句法联合训练，tagger预测的词的embedding作为parser的输入，parser用的是BIST parser (K&G)，PTB的LAS结果是92.87（我跑出来的是94.38），比BIST parser提升1.5+，进一步在61种Universal
% Dependencies treebanks，比UDPipe作为baseline高了3.6}


% the main idea of Stack-Discrete is using the discrete POS tags predicted by the tagger as extra features in the parser. Assuming $p_1p_2, \ldots p_n$ are the produced POS tag sequence, we represent each $i^{th}$ POS tag by a POS embedding $\mathbf{e}_i^p$, and then concatenate it to $x_i$ to enhance the input representation of parser:
% \begin{equation}
% \mathbf{x}_i=\mathbf{e}_i^w \oplus \mathbf{e}_i^c \oplus \mathbf{e}_i^p
% \end{equation}

%Except for the shared input word representations, the tagger uses a encoder independent of parser in this framework.

\paragraph{Stack.}
% The key difference between {{Stack}} and {{Stack-Discrete}} is that, rather than using discrete 1-best POS tag,
The \textit{Stack} takes BiLSTM hidden outputs of the tagger, denoted as $\mathbf{r}_i^p$, as the extra input of the parser.
In this way, the error propagation problem can be better handled.
\begin{equation}
% \mathbf{x}_i=\mathbf{e}_i^w \oplus \mathbf{e}_i^c \oplus \mathbf{r}_i^p
\mathbf{x}^{parse}_i = \mathbf{x}_i \oplus \mathbf{r}_i^p
\end{equation}
%aiming to solve the error propagation problem. We borrow
The idea of the \textit{Stack} joint method is mainly borrowed from \citet{zhang-weiss-2016-stack}.
They propose the \emph{stack-propagation} approach to avoid using explicit POS tags in dependency parsers.
They employ the simple feed-forward networks for both tagging and parsing \cite{chen2014fast}.
Without BiLSTM encoders, they use the hidden outputs of a single-layer MLP of the tagging component as extra inputs of the parsing component.

\paragraph{Training loss.} During training, we directly add together all losses of different tasks, i.e., the parsing loss, the homogeneous POS tagging loss, and the heterogeneous POS tagging loss. %twe finally obtain the homogeneous tagging loss $\mathcal{L}_{\mathrm{POS}}$, the heterogeneous tagging loss $\mathcal{L}_{\mathrm{POS^\prime}}$, and the parsing loss $\mathcal{L}_{\mathrm{ARC}}$ and $\mathcal{L}_{\mathrm{REL}}$, we take the sum of them as our training loss
\begin{equation}
\mathcal{L}=\mathcal{L}_{\mathrm{DEP}}+\mathcal{L}_{\mathrm{POS}}+\mathcal{L}_{\mathrm{POS^\prime}}
\end{equation}

==> source code/content/related_work.tex <==
\section{Related Works}

Previous studies \cite{mcdonald-d11-delexicalized,lei-etal-2014-low} show POS tags are indispensable ingredients for composing different features in the traditional pre-DL dependency parsers \cite{koo-acl10-3o,zhang-nivre-p11-transition}.
% \citet{mcdonald-d11-delexicalized} show that their full parser achieves with all features obtains an UAS of 89.3, whereas
% a delexicalized parser with only nonlexical features obtains an UAS of 82.5 on the English dataset of the CoNLL-2007 shared task, indicating that
% that POS tags contain a
% significant amount of information for dependency parsing.
Meanwhile, \citet{li-etal-2011-joint} show that the error propagation problem introduced by predicted POS tags degrades parsing accuracy by about 6 (UAS) on different Chinese  datasets.
Therefore, researchers propose to jointly model the POS tagging and dependency tasks in the graph-based \cite{li-etal-2011-joint} and transition-based \cite{hatori-etal-2011-incremental} %(), and easy-first parsing
frameworks, leading to promising results.
The key challenge is to define scoring functions on the joint results, and design effective search algorithms to determine optimal joint answers in the enlarged search space.
Furthermore, joint models of word segmentation, POS tagging, and parsing are also proposed \cite{hatori-EtAl:2012:ACL2012}.

In the DL era, joint modeling of multiple related tasks becomes much easier under the MTL framework \cite{collobert-08-multi-task}.
In fact, MTL has become an extensively used and powerful technique for many problems.
The basic idea is sharing the encoder part while using separate decoders for different tasks.
The major advantages of employing MTL are two-fold, i.e., 1) exploiting the correlation and mutual helpfulness among related tasks, and 2) making direct use of all (usually non-overlapping) labeled data of different tasks.
The Share-Light and Share-Tight methods are both typical MTL frameworks, and the main difference lies in the amount of shared parameters.
Actually, there are still many other variants due to the flexibility of MTL.
For example, \citet{straka-2018-udpipe} stacks task-specific private BiLSTMs over shared BiLSTMs for joint tagging and parsing.
Based on the current results, we expect that such variants may achieve very similar performance.

% The Stack-Discrete method investigated in this work is borrowed from   \citet{nguyen-verspoor-2018-improved}, who first propose to jointly model  POS tagging and dependency parsing by 1) stacking two BiLSTM encoders and 2) using the embeddings of online predicted 1-best POS tags as extra inputs of the BiLSTM encoder of the parsing component.
% They implement this idea based on the BIST parser  \cite{kiperwasser-goldberg-2016-simple} and report large improvement.
% In this work, we use the {Stack-Discrete} joint method as a representative approach and try to make thorough investigations based on the state-of-the-art biaffine parser.

The \textit{Stack} method is similar to the \emph{stack-propagation} method of \citet{zhang-weiss-2016-stack}.
Their basic idea is to use the hidden outputs of the POS tagging components as extra inputs of the parsing components, forming a stacked structure.
During training, parsing loss is directly propagated into the full tagging component whereas tagging loss only indirectly influences the parsing components via their shared parts.
%the \textbf{stack-propagation}  to avoid using explicit POS tags in dependency parsers.
Their pioneer work employ a simple feed-forward network for both tagging and parsing \cite{chen2014fast}, and only achieves an LAS of 91.41 on PTB.   %Without BiLSTM encoders, they use the hidden outputs of a single-layer MLP of the tagging component as extra inputs of the parsing component.
Another inspiring work related with the \textit{Stack} method is \citet{hashimoto-etal-2017-joint}, who propose to jointly train many tasks of different complexity in a very deep and cascaded network architecture, where higher levels are used for more complex tasks.

%aiming to solve the error propagation problem. We borrow

%and achieve a final LAS of 91.41.
%Joint models.
%POS tagging and parsing are too closely related: parsing is a superset task of POS tagging. Not equally-positioned tasks.
%Joint POS tagging and parsing.
%Even word segmentation.

% Multi-task learning approaches.

% Stack-propgagtion. Vietanam. (stack-soft)

% \cite{clark-etal-2018-semi}是否要写到这？只用了word embedding


%share-loose share-tight \cite{straka-2018-udpipe}
% UDpipe2.0引用一下

% 越南人stack-hard

%\citet{dozat-etal-2017-stanfords} first perform left-to-right LSTM over word characters and add together word embedding and \textsc{CharLSTM} word representation, which is also adopted in the BiLSTM-CRF named entity recognition system \cite{lample-etal-2016-neural}.
%\citet{che-etal-2018-towards} use the sum of word embedding, \textsc{CharLSTM} word representation, and ELMo output word representation \cite{peters-2018-elmo}.
%ELMo \cite{peters-2018-elmo} applies convolution neural network on word characters and use charCNN word representation as inputs without using word embedding.
%\citet{kitaev-klein-2018-constituency} find that concatenating （是否是concate?) \textsc{CharLSTM} word representation with word embedding performs better than concatenating POS tag embedding with word embedding in English??? (需要确认是否只有英语） constituency parsing based on self-attention encoding. % They also find that further removing word embedding does not hurt performance? (根据我们的实验结果考虑是否写）
% 找一下利用CNN做char-based word represeantion的工作


% 无监督句法分析通常假设给定正确的词性标注。其实目前一些无监督句法分析已经打破了这个限制（问一下tukewei老师）？


%多个任务同时做，包括POS、NE、chunking, parsing. 日本人


% 特别想找到那篇文章，说明只使用词特征，而不是用词性特征，性能急剧下降。
% 找到啦！
% https://www.aclweb.org/anthology/D11-1006
%  For example, when training and testing a parser on our English data, a parser
% with all features obtains an UAS of 89.3 whereas
% a delexicalized parser – a parser that only has nonlexical features – obtains an UAS of 82.5. The
% key observation is that part-of-speech tags contain a
% significant amount of information for unlabeled dependency parsing.

%  dependency model with valence (DMV) of Klein
% and Manning (2004),

% Unsupervised


==> source code/content/use_bert.tex <==
\section{Integration with BERT}

\begin{table*}[htb]
\centering
\begin{tabular}{l|rrr|rrrr}
\toprule
Dataset & \#Train & \#Dev & \#Test & \#tokens & \#chars & \#POS & \#labels \\\\[-12pt]
\hline\\[-10pt]
PTB & 39,832 & 1,700 & 2,416 & 44,389 & 79 & 45 & 45 \\
CoNLL09 & 22,277 & 1,762 & 2,556 & 40,878 & 4,243 & 41 & 41 \\
CTB7 & 46,427 & 2,079 & 2,796 & 55,324 & 4,595 & 35 & 46 \\\\[-12pt]
\hline\\[-10pt]
PKU & 1,208,850 & 2,000 & 3,000 & 267,943 & 6,488 & 63 & - \\
\bottomrule
\end{tabular}
\caption{The statistics of dependency parsing and heterogeneous POS Tagging corpora.}
\label{table:statistics}
\end{table*}

Recently, the development of contextual word representations such as ELMo \cite{peters-2018-elmo} and BERT \cite{devlin-etal-2019-bert} have dramatically showed great success for many natural language processing (NLP) tasks.
Taking BERT as an example, their main idea is to train a multi-layer bidirectional Transformer \cite{vaswani-2017-attention} encoder on large-scale unlabeled texts, and use it to produce pretrained language representations.

In this paper, we take BERT as a new representation to enhance the current input features.
Since both our tagging and parsing tasks adopt word-level features, while BERT uses a more fine-grained input (subwords for English and characters for Chinese), this shows a little mismatch.
We have tried three ways: take 1) the first one, 2) the last one, 3) the average of all pieces in a word as a summary of them.
Results show that the average strategy is slightly better than the other two ways.

\citet{devlin-etal-2019-bert} compared two strategies for applying BERT to downstream tasks: the feature integration method and the finetune method, and recommended the later one.
Since what we explored are both word-level tasks, we adopt a combination of the two strategies.
Besides classifiers, we retain the word embedding and BiLSTM encoders, and feed BERT as extra feature into the BiLSTM layer.
Meanwhile, we do not freeze parameters of BERT, but finetune them during training.
Since the parameter space of BERT is huge, using it crudely can easily fall into overfitting, we apply series of regularization strategies to help improve the performance.

\subsubsection{Token Dropout} During the pretraining procedure, \citet{devlin-etal-2019-bert} introduced a so-called ``Masked LM'' strategy, which replaces the word piece with a special token randomly with a certain probability.
We retain this method at the finetuning stage \cite{Kondratyuk201975L1,clark-etal-2018-semi}.
Such special dropout strategy aims to force the model to learn a distributional contextual representation of every input token, which is critical to prevent model from overfitting and can effectively improve test performance.

\subsubsection{Layer Attention} Rather than restricted to any sublayers, we tend to collapse all BERT layers into a single vector by weighted-summation \cite{peters-2018-elmo,Kondratyuk201975L1}, called layer attention.
Specifically, assuming the intermediate output of $i^{th}$ token at $j^{th}$ BERT layer is $\mathbf{h}_{ij}$, we combine the total $L=12$ layers in the following way:
\begin{equation}
\mathbf{bert}_i^{task}=\gamma^{task}\sum_{j=1}^{L}{\mathrm{softmax}\left(\mathbf{s}_j^{task} \right) \cdot \mathbf{h}_{ij}}
\end{equation}
where $\gamma^{task}$ and $\mathbf{s}_j^{task}$ are task specific trainable weights.
We also randomly set $\mathbf{s}_j^{task}$ to $-\infty$, i.e., discard some layers to prevent the model from focusing too much on a single layer.
Once getting the BERT feature, we modify Equation \ref{eq:input} to
\begin{equation}
\mathbf{x}_i=\mathbf{e}_{w_i}^w \oplus \mathbf{bert}_i^{task}
\end{equation}
in which the tagger and parser acquire different representations, since they use separate weights corresponding to all BERT layers, and the softmax-normalized values indicate that, compared with parsing, the tagging task prefers the front layers.
Note that we directly replace the character-level model with BERT since we found the information learned by BERT has been enough and use them simultaneously doesn't make the results better.

==> source code/figures/instance.tex <==
\begin{figure}[tb]
\centering
\begin{dependency}[arc edge, arc angle=80, text only label, label style={above}]
\begin{deptext} [row sep=0.025cm, column sep=0.1cm]
\$ \& 中央台 \& 驻  \& 香港 \& 记者 \& 报道 \&。 \\
\& CCTV \& in  \& HK \& journalist \& reports \&.  \\
CTB: \& \texttt{NR} \& \texttt{VV} \& \texttt{NR} \& \texttt{NN} \& \texttt{VV} \& \texttt{PU} \\
PKU: \& \texttt{jn} \& \texttt{vt} \& \texttt{ns} \& \texttt{n}  \& \texttt{vt} \& \texttt{w}  \\
\end{deptext}
\depedge[edge style={black}]{5}{2}{\color{black}nn}
\depedge[edge style={black}]{5}{3}{\color{black}rcmod}
\depedge[edge style={black}]{3}{4}{\color{black}dobj}
\depedge[edge style={black}]{6}{5}{\color{black}nsubj}
\depedge[edge style={black}]{1}{6}{\color{black}root}
\depedge[edge style={black}]{6}{7}{\color{black}punct}
\end{dependency}

\caption{An example dependency tree with both homogeneous (CTB) and heterogeneous (PKU) POS tags.}
\label{fig:example-dep}
\end{figure}

==> source code/tables/dev.tex <==
% \begin{table}[tb]
% \centering
\begin{tabular}{llccc}
\toprule
& & PTB & CoNLL09 & CTB7 \\\\[-12pt]
% \hline\\[-10pt]
% & Basic ($e_w \oplus e_c$) & 93.97 & 86.09 & 85.23 \\\\[-12pt]
\hline\\[-10pt]
\multirow{3}{*}{\shortstack{homo}}
& \textit{Share-Loose}    &         93.95  &         86.28  &         85.56  \\
& \textit{Share-Tight}    &         93.93  &         86.17  &         85.56  \\
& \textit{Stack}          & \textbf{94.09} & \textbf{86.26} & \textbf{85.79} \\\\[-9pt]
\hline\\[-7pt]
\multirow{3}{*}{\shortstack{hetero}}
& \textit{Share-Loose}    & - &         86.05  &         85.62  \\
& \textit{Share-Tight}    & - & \textbf{86.25} &         85.76  \\
& \textit{Stack}          & - &         86.16  & \textbf{85.86} \\\\[-9pt]
\hline\\[-7pt]
\multirow{3}{*}{\shortstack{homo\\+\\hetero}}
& \textit{Share-Loose}    & - &         86.30  &         85.57  \\
& \textit{Share-Tight}    & - &         86.62  &         85.86  \\
& \textit{Stack}          & - & \textbf{86.69} & \textbf{85.88} \\
\bottomrule
\end{tabular}
% \caption{Parsing performance (LAS) comparison on the dev data for the three joint methods.}
% \label{table:dev}
% \end{table}


% \begin{table*}[tb]
%   \centering
%   \begin{tabular}{llccccccccc}
%   \hline
%   & & \multicolumn{3}{c}{PTB} & \multicolumn{3}{c}{CoNLL09} & \multicolumn{3}{c}{CTB7} \\
%   & & TA & UAS & LAS & TA & UAS & LAS & TA & UAS & LAS \\
%   \hline
%   \multicolumn{2}{c}{Baseline ($e_w \oplus e_c$)} & \textbf{97.58} & 95.78 & 93.97 & 96.59 & 88.98 & 86.09 & 96.72 & 88.35 & 85.23 \\
%   \hline
%   \multirow{4}{*}{\specialcell{ w/ homo tagging \\ $\mathcal{L}_{DEP} + \mathcal{L}_{POS}$}}
%   & Share-Loose & 97.41 & 95.72 & 93.95 & 96.52 & 89.25 & 86.28 & 96.68 & 88.63 & 85.56 \\
%   & Share-Tight & 97.51 & 95.73 & 93.93 & 96.64 & 89.09 & 86.17 & 96.67 & 88.58 & 85.56 \\
%   &  Stack-Discrete & 97.02 & 95.70 & 93.86 & 96.61 & 89.32 & 86.35 & 96.75 & 88.51 & 85.49 \\
%   &  Stack & 97.54 & \textbf{95.86} & \textbf{94.09} & 96.57 & 89.13 & 86.26 & 96.68 & 88.81 & 85.79 \\
%   \hline
%   \multirow{4}{*}{\specialcell{w/ homo \& hetero tagging \\ $\mathcal{L}_{DEP}+ \mathcal{L}_{POS}+ \mathcal{L}_{POS'} $  }}
%   & Share-Loose & - & - & - & 96.82 & 89.22 & 86.30 & \textbf{96.90} & 88.63 & 85.57 \\
%   & Share-Tight    & - & - & - & 96.84 & 89.45 & 86.62 & 96.82 & \textbf{88.84} & 85.86 \\
%   &  Stack-Discrete    & - & - & - & 96.82 & 89.31 & 86.46 & 96.85 & 88.75 & 85.85 \\
%   &  Stack    & - & - & - & \textbf{96.84} & \textbf{89.50} & \textbf{86.69} & 96.83 & 88.80 & \textbf{85.88} \\
%   \hline
%   \end{tabular}
%   \caption{Results on the dev data of the three datasets. We report the POS Tagging Accuracies (TA), UAS and LAS of all model variants, respectively.
% }
%   \label{table:dev}
% \end{table*}

==> source code/tables/final.tex <==
\begin{table}[tb]
\setlength{\tabcolsep}{1.5pt}
\begin{widepage}
\centering
\begin{tabular}{llccccccccc}
\toprule
& & \multicolumn{3}{c}{PTB} & \multicolumn{3}{c}{CoNLL09} & \multicolumn{3}{c}{CTB7} \\
& & TA & UAS & LAS & TA & UAS & LAS & TA & UAS & LAS \\\\[-12pt]
\hline\\[-10pt]
\multirow{7}{*}{w/o BERT}
& \citet{andor-etal-2016-global} & 97.44 & 94.61 & 92.79 & - & 84.72 & 80.85 & - & - & - \\
& \citet{Timothy-d17-biaffine} & 97.3\,\,\,  & 95.74 & 94.08 & - & 88.90 & 85.38 & - & - & - \\
& \citet{ji-etal-2019-graph} & 97.3\,\,\,  & 95.97 & 94.31 & - & - & - & - & - & - \\
%  & \citet{Timothy-d17-biaffine} (our impl) & 95.89 & 94.22 & 88.69 & 85.53 & 88.20 & 84.90 \\
& \citet{li-etal-2019-attentive} & 97.3\,\,\,  & 95.93 & 94.19 & - & 88.77 & 85.58 & - & - & - \\
& Basic ($\mathbf{e}^w \oplus \mathbf{e}^c$) & 97.50 & 95.97 & 94.34 & 96.42 & 89.12 & 86.00 & 96.48 & 88.58 & 85.40 \\
& Pipeline ($\mathbf{e}^w \oplus \mathbf{e}^c \oplus \mathbf{e}^p$) & 97.50 & 95.88 & 94.27 & 96.42 & 89.12 & 85.98 & 96.48 & 88.42 & 85.28 \\
& \textit{Stack} & \textbf{97.91} & \textbf{96.13} & \textbf{94.53} & 96.55 & 89.46 & 86.44 & 96.62 & 88.86 & 85.88 \\
& \textit{Stack} w/ hetero & - & - & - & \textbf{96.66} & \textbf{89.85} & \textbf{86.85} & \textbf{96.72} & \textbf{89.26} & \textbf{86.27} \\\\[-12pt]
\hline\\[-10pt]
\multirow{4}{*}{w/ BERT}
& \citet{li-etal-2019-attentive} & - & 96.67 & 95.03 & - & 92.24 & 89.29 & - & - & - \\
& Basic ($\mathbf{e}^w \oplus \mathbf{e}^c$) & 97.42 & 96.85 & 95.14 & 97.29 & 92.21 & 89.42 & 97.22 & 91.66 & 88.75 \\
& \textit{Stack}  & \textbf{97.57} & \textbf{96.85} & \textbf{95.25} & 97.36 & 92.44 & 89.68 & 97.32 & 91.67 & 88.84 \\
& \textit{Stack} w/ hetero & - & - & - & \textbf{97.39} & \textbf{92.46} & \textbf{89.76} & \textbf{97.40} & \textbf{91.81} & \textbf{89.04} \\
\bottomrule
\end{tabular}
\end{widepage}
\caption{Final results on the test data. It is noteworthy that we produce our experiments with single run for each model on each dataset, since our preliminary experiments that we train \textit{Stack} w/ hetero and Basic on CTB7 for four times show the variance of performances is small ($\sigma^2 < 0.01$). }
\label{table:final-results}
\end{table}
% \begin{table*}[hbt]
%   \centering
%   \begin{tabular}{llcccccc}
%   \hline
%   & & \multicolumn{2}{c}{PTB} & \multicolumn{2}{c}{ CoNLL09} & \multicolumn{2}{c}{CTB7} \\
%   & & UAS & LAS & UAS & LAS & UAS & LAS \\
%   \hline
%   \multirow{7}{*}{w/o BERT}
%   & \citet{andor-etal-2016-global} & 94.61 & 92.79 & 84.72 & 80.85 & - & - \\
%   & \citet{Timothy-d17-biaffine} & 95.74 & 94.08 & 88.90 & 85.38 & - & - \\
%   & \citet{ji-etal-2019-graph} & 95.97 & 94.31 & - & - & - & - \\
% %  & \citet{Timothy-d17-biaffine} (our impl) & 95.89 & 94.22 & 88.69 & 85.53 & 88.20 & 84.90 \\
%   & \citet{li-etal-2019-attentive} & 95.93 & 94.19 & 88.77 & 85.58 & - & - \\
%   & Basic ($\mathbf{e}^w \oplus \mathbf{e}^c$) & 95.97 & 94.34 & 89.12 & 86.00 & 88.54 & 85.34 \\
%   & Pipeline ($\mathbf{e}^w \oplus \mathbf{e}^c \oplus \mathbf{e}^p$) & 95.88 & 94.27 & 89.12 & 85.98 & 88.42 & 85.28 \\
%   & Joint Stack w/ homo tags & \textbf{96.13} & \textbf{94.53} & 89.46 & 86.44 & 88.86 & 85.88 \\
%   & Joint Stack w/ homo \& hetero tags & - & - & \textbf{89.85} & \textbf{86.85} & \textbf{89.21} & \textbf{86.22} \\
%   \hline
%   \multirow{4}{*}{w/ BERT}
%   & \citet{li-etal-2019-attentive} & 96.67 & 95.03 & 92.24 & 89.29 & - & - \\
%   & Basic ($\mathbf{e}^w \oplus \mathbf{e}^c \oplus \mathbf{r}^{BERT}$) & 96.85 & 95.14 & 92.21 & 89.42 & 91.66 & 88.75 \\
%   & Joint Stack w/ homo tags & \textbf{96.85} & \textbf{95.25} & 92.44 & 89.68 & 91.67 & 88.84 \\
%   & Joint Stack w/ homo \& hetero tags & - & - & \textbf{92.46} & \textbf{89.76} & \textbf{91.81} & \textbf{89.04} \\
%   \hline
%   \end{tabular}
%   \caption{Final results of the model on test sets of PTB, CoNLL09 and CTB7.}
%   \label{table:final-results}
% \end{table*}

==> source code/tables/statistics.tex <==
\begin{table}[tb]
\centering
% \setlength{\tabcolsep}{5pt}
\begin{tabular}{l|rrr|cc}
\toprule
& \#Train & \#Dev & \#Test & \#POS & \#labels \\\\[-12pt]
\hline\\[-10pt]
PTB & 39,832 & 1,700 & 2,416 & 45 & 45 \\
CoNLL09 & 22,277 & 1,762 & 2,556 & 41 & 41 \\
CTB7 & 46,427 & 2,079 & 2,796 & 35 & 46 \\\\[-12pt]
\hline\\[-10pt]
PKU & 1,208,850 & 2,000 & 3,000 & 63 & - \\
\bottomrule
\end{tabular}
\caption{Data statistics, including numbers of sentences, POS tags, and dependency labels.}
\label{table:statistics}
\end{table}

% \begin{table}[htb]
%   \centering
%   \begin{tabular}{l|rrr|rrrr}
%   \hline
%   Dataset & \#Train & \#Dev & \#Test & \#tokens & \#chars & \#POS & \#labels \\
%   \hline
%   PTB & 39,832 & 1,700 & 2,416 & 44,389 & 79 & 45 & 45 \\
%   CoNLL09 & 22,277 & 1,762 & 2,556 & 40,878 & 4,243 & 41 & 41 \\
%   CTB7 & 46,427 & 2,079 & 2,796 & 55,324 & 4,595 & 35 & 46 \\
%   \hline
%   PKU & 1,208,850 & 2,000 & 3,000 & 267,943 & 6,488 & 63 & - \\
%   \hline
%   \end{tabular}
%   \caption{Data statistic, including numbers of sentences, POS tags, and dependency labels.}
%   \label{table:statistics}
% \end{table}


==> source code/tables/tag-dev.tex <==
% \begin{table}[tb]
% \centering
\begin{tabular}{lcccccc}
\toprule
& PTB & CoNLL09 & CTB7 \\\\[-12pt]
\hline\\[-10pt]
$\mathbf{e}^p$ & 87.79 & 75.94 & 75.72 \\
$\mathbf{e}^w$ & 93.42 & 85.30 & 84.43 \\
$\mathbf{e}^c$ & 93.34 & 84.42 & 83.73 \\\\[-12pt]
\hline\\[-10pt]

$\mathbf{e}^w \oplus \mathbf{e}^p$ & 93.92 & 85.94 & 85.12 \\

$\mathbf{e}^w \oplus \mathbf{e}^c$ & \textbf{93.97} & 86.09 & 85.23 \\\\[-12pt]
\hline\\[-10pt]
$\mathbf{e}^w \oplus \mathbf{e}^c \oplus \mathbf{e}^p$ & 93.88 & \textbf{86.17} & \textbf{85.32} \\
$\mathbf{e}^w \oplus \mathbf{e}^c \oplus \mathbf{e}^p \oplus \mathbf{e}^{p\prime}$ & - & 86.01 & 85.23 \\
\bottomrule
\end{tabular}
% \caption{Parsing performance (LAS) on the dev data under the pipeline framework. $\mathbf{e}^w \oplus \mathbf{e}^c$ is our basic model.}
% \label{table:tag-dev}
% \end{table}


% \begin{table}[tbh]
%   \setlength{\tabcolsep}{0.3pt}
%   \centering
%   \begin{tabular}{lcccccc}
%   \hline
%   & \multicolumn{2}{c}{PTB} & \multicolumn{2}{c}{CoNLL09} & \multicolumn{2}{c}{CTB7} \\
%   & UAS & LAS & UAS & LAS & UAS & LAS \\
%   \hline
%   $\mathbf{e}^p$ & 90.56 & 87.79 & 80.18 & 75.94 & 79.50 & 75.72 \\
%   $\mathbf{e}^w$ & 95.46 & 93.42 & 88.46 & 85.30 & 87.93 & 84.43 \\
%   $\mathbf{e}^c$ & 95.25 & 93.34 & 87.72 & 84.42 & 87.20 & 83.73 \\
%   \hline

%   $\mathbf{e}^w \oplus \mathbf{e}^p$ & 95.69 & 93.92 & 88.80 & 85.94 & 88.20 & 85.12 \\
%   \hline
%   $\mathbf{e}^w \oplus \mathbf{e}^c$ $[\star]$ & \textbf{95.78} & \textbf{93.97} & 88.98 & 86.09 & \textbf{88.35} & 85.23 \\
%   $\mathbf{e}^w \oplus \mathbf{e}^c \oplus \mathbf{e}^p$ & 95.66 & 93.88 & \textbf{89.11} & \textbf{86.17} & 88.34 & \textbf{85.32} \\
%   $\mathbf{e}^w \oplus \mathbf{e}^c \oplus \mathbf{e}^p \oplus \mathbf{e}^{p\prime}$& - & - & 88.97 & 86.01 & 88.26 & 85.23 \\
%   \hline
%   \end{tabular}
%   \caption{Results of dependency parsing on dev data by utilizing POS tags in different ways. The row marked by $[\star]$ are results of our baseline. 在ctb7和conll上的规律不一致：dense vs. sparse}
%   \label{table:tag-dev}
% \end{table}

==> source code/tables/tag-pair.tex <==
\begin{table}[tb]
% \setlength{\tabcolsep}{2.5pt}
\centering
\begin{tabular}{rlcc||rlcc}
\toprule
& & UAS & LAS & & & UAS & LAS \\\\[-12pt]
\hline\\[-10pt]
\texttt{NN} & $\rightarrow$ \texttt{NN} & 91.73 & 89.69 & \texttt{NR}  & $\rightarrow$ \texttt{NR}  & 91.73 & 86.96 \\
            & $\rightarrow$ \texttt{VV} & 67.25 & 44.98 &              & $\rightarrow$ \texttt{NN}  & 86.39 & 83.67 \\
            & $\rightarrow$ \texttt{NR} & 90.43 & 86.96 & \texttt{JJ}  & $\rightarrow$ \texttt{JJ}  & 95.40 & 94.33 \\
            & $\rightarrow$ \texttt{JJ} & 91.96 & 20.54 &              & $\rightarrow$ \texttt{NN}  & 92.82 & 14.92 \\
\texttt{VV} & $\rightarrow$ \texttt{VV} & 85.92 & 84.12 & \texttt{DEG} & $\rightarrow$ \texttt{DEG} & 96.75 & 95.91 \\
            & $\rightarrow$ \texttt{NN} & 65.60 & 40.07 &              & $\rightarrow$ \texttt{DEC} & 92.06 & 26.56 \\
            & $\rightarrow$ \texttt{VA} & 84.75 & 83.05 & \texttt{DEC} & $\rightarrow$ \texttt{DEC} & 94.28 & 92.39 \\
            & $\rightarrow$ \texttt{AD} & 55.32 & 25.53 &              & $\rightarrow$ \texttt{DEG} & 96.88 & 22.22 \\
\bottomrule
\end{tabular}
\caption{The impact of specific POS tagging error patterns on parsing.}
\label{table:tag-pair}
\end{table}

==> tables/statistics.tex <==
\begin{table}[tb]
\centering
% \setlength{\tabcolsep}{5pt}
\begin{tabular}{l|rrr|cc}
\toprule
& \#Train & \#Dev & \#Test & \#POS & \#labels \\\\[-12pt]
\hline\\[-10pt]
PTB & 39,832 & 1,700 & 2,416 & 45 & 45 \\
CoNLL09 & 22,277 & 1,762 & 2,556 & 41 & 41 \\
CTB7 & 46,427 & 2,079 & 2,796 & 35 & 46 \\\\[-12pt]
\hline\\[-10pt]
PKU & 1,208,850 & 2,000 & 3,000 & 63 & - \\
\bottomrule
\end{tabular}
\caption{Data statistics, including numbers of sentences, POS tags, and dependency labels.}
\label{table:statistics}
\end{table}

% \begin{table}[htb]
%   \centering
%   \begin{tabular}{l|rrr|rrrr}
%   \hline
%   Dataset & \#Train & \#Dev & \#Test & \#tokens & \#chars & \#POS & \#labels \\
%   \hline
%   PTB & 39,832 & 1,700 & 2,416 & 44,389 & 79 & 45 & 45 \\
%   CoNLL09 & 22,277 & 1,762 & 2,556 & 40,878 & 4,243 & 41 & 41 \\
%   CTB7 & 46,427 & 2,079 & 2,796 & 55,324 & 4,595 & 35 & 46 \\
%   \hline
%   PKU & 1,208,850 & 2,000 & 3,000 & 267,943 & 6,488 & 63 & - \\
%   \hline
%   \end{tabular}
%   \caption{Data statistic, including numbers of sentences, POS tags, and dependency labels.}
%   \label{table:statistics}
% \end{table}

